Bose-Einstein Condensation and Kinetic energy of liquid $^3$He-$^4$He Mixtures

We present neutron scattering measurements of the momentum distribution of liquid ${^3}$He-${^4}$He mixtures. The experiments were performed at wavevectors $Q$, 26 $\leq$ $Q$ $\leq$ 29 {\AA$^{-1}$}, on the MARI time-of-flight spectrometer at the ISIS Facility, Rutherford Appleton Laboratory, a spallation neutron source. Mixtures with $^3$He concentrations $x$ between 0 and 20% were investigated both in the superfluid and normal phases. From the data, we extract the Bose-Einstein condensate fraction $n_0$ and the momentum distributions of $^3$He and $^4$He atoms. We find that $n_0$ increases somewhat above the pure $^4$He value when $^3$He is added; e.g from $n_0=(7.25\pm0.75)%$ at $x=$ 0 to $(11\pm3)%$ at $x=$ 15-20%. This agrees with predictions but is less than the only previous measurement. We find a $^4$He kinetic energy $K_4$ for pure $^4$He that agrees with previous determinations. $K_4$ decreases somewhat with increasing $^3$He concentration, less than observed previously and found in early calculations but in agreement with a more recent Monte Carlo calculation. The $^3$He response is not well reproduced by a Fermi gas momentum distribution, $n(\bf{k})$. Rather an $n(\bf{k})$ having a small step height at the Fermi surface and a substantial high momentum tail characteristic of a strongly interacting Fermi liquid provides a good fit. This $n(\bf{k})$ is consistent with calculated $n(\bf{k})$. Thus agreement between theory and experiment is obtained comparing $n(\bf{k})$ in contrast to earlier findings based on comparing calculated and observed $^3$He kinetic energies.

==> 3_4email <==
 Dear Henry,
  I would agree with you that the fig#4 with fits to experimental values
looks better than the other figures, specially when it is followed by
fig15b. where we show a relative agreement with PIMC results.

 Thank you very much for sending in the corrections by fax. I have made
the recommended changes.

 I have also made a slight change in the second paragraph of section 
IV.A.2
(5th to 6th lines) as follows:  I have removed "\eta=0" because it
introduces a singularity in equation 12. and corresponds to a non defined
 J_IA in equation 13. Strictly  speaking, I simply fixed H=1 and the
constraint lead to H_F~0 and the effect of eta in the fits becomes
irrelevant.



